Semantic Environment Atlas for Object-Goal Navigation

In this paper, we introduce the Semantic Environment Atlas (SEA), a novel mapping approach designed to enhance visual navigation capabilities of embodied agents. The SEA utilizes semantic graph maps that intricately delineate the relationships between places and objects, thereby enriching the navigational context. These maps are constructed from image observations and capture visual landmarks as sparsely encoded nodes within the environment. The SEA integrates multiple semantic maps from various environments, retaining a memory of place-object relationships, which proves invaluable for tasks such as visual localization and navigation. We developed navigation frameworks that effectively leverage the SEA, and we evaluated these frameworks through visual localization and object-goal navigation tasks. Our SEA-based localization framework significantly outperforms existing methods, accurately identifying locations from single query images. Experimental results in Habitat scenarios show that our method not only achieves a success rate of 39.0%, an improvement of 12.4% over the current state-of-the-art, but also maintains robustness under noisy odometry and actuation conditions, all while keeping computational costs low.

==> defs.tex <==
\usepackage{chngcntr}
\usepackage{titlesec}

% Environment for review comments
\newcounter{revcomcounter}[section]
\renewcommand{\therevcomcounter}{\arabic{section}.\arabic{revcomcounter}}

% Review comment environment
\newenvironment{revcom}[1][]{%
    \refstepcounter{revcomcounter}%
    \ifx\\#1\\%
    \else
        \label{#1}%
    \fi
    \begin{trivlist}\item\textbf{Comment~\therevcomcounter: }\em%
        }%
        {\end{trivlist}}%

% Environment for responding to review comments
\newenvironment{response}[1][]{%
    \begin{trivlist}\item\textbf{Response: }%
        }%
        {\end{trivlist}}%

% Reset comment counter in each section
\counterwithin*{revcomcounter}{section}

% Define section format without numbers
\titleformat{\section}{\normalfont\large\bfseries}{}{0em}{}

==> fig/SEA.tex <==
\begin{figure*}[t!]
\centering
\begin{minipage}{\textwidth}{
\centering
{\centering\includegraphics[width=\textwidth]{fig/SEA_.pdf}}
\centering
\caption{
{Adaptive SEA update procedure.}
% 
% The semantic prior graph and episodic graph are used to update the prior information. 
% 
% The semantic prior graph is updated by extracting place-object and place connections from episodic graphs.
% 
}
\label{fig:SEA}}
\end{minipage}
\end{figure*}


==> fig/cluster_2azQ1b91cZZ.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig/cluster_2azQ1b91cZZ_.pdf}}\centering
\caption{{Visualization of place clusters on the map in a test environment (\textit{2azQ1b91cZZ}) of MP3D}}
\label{fig:cluster_2azQ1b91cZZ}
\end{figure*}

==> fig/cluster_41.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig/cluster_41_.pdf}}\centering
\caption{{Visualization of a place cluster ($P_{41}$) on the maps in 11 test environments of MP3D}}
\label{fig:cluster_41}
\end{figure*}

==> fig/cluster_zsNo4HB9uLZ.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig/cluster_zsNo4HB9uLZ_.pdf}}\centering
\caption{{Visualization of place clusters on the map in a test environment (\textit{zsNo4HB9uLZ}) of MP3D}}
\label{fig:cluster_zsNo4HB9uLZ}
\end{figure*}

==> fig/episodic_graph_example.tex <==
\begin{figure*}[t!]{\centering\includegraphics[height=0.85\textheight]{fig/episodic_graph_example_withobj_v2.pdf}}\centering
\caption{
\textbf{Example of constructing an episodic graph.}
While randomly investigating the surroundings, the agent accumulates an episodic graph. A place graph, an image graph, and an object graph comprise an episodic graph.
% 
Color on the image node indicates the place cluster, circles indicate image nodes, and triangles represent object nodes.
% % 
% The reachability and connectedness between places and objects are collected when exploring. 
% % 
% If the place clusters of two connected image nodes changes, the two place clusters are connected.
% % 
% For example, when t=100, the agent moves from the bedroom (blue) to the kitchen (purple).
% % 
% The reachability between the blue and purple place clusters is one. 
% % 
% The topological semantic graph can obtain connectedness between nodes Without utilizing pose information.
% % 
% Top-down maps and node positions are only used for visualization and are not used to construct a graph.
}
\label{fig:episodic_graph_example}
\end{figure*}

==> fig/episodic_graph_example_last.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=0.8\textwidth]{fig/episodic_graph_example_last_v2.pdf}}\centering
\caption{{Visualization of episodic graphs on various training environments.}}
\label{fig:episodic_graph_example_last}
\end{figure*}

==> fig/episodicgraph.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig/semanticgraphmap_.pdf}}\centering\squeezelittle
\caption{
\textbf{Construction of semantic graph map.}
% 
By integrating the current observation and the previous semantic graph map (SGM; $E_{t-1}$), the graph map is updated. 
% 
If it is discovered that the current location differs from the previous location, an image node is added to the graph. 
% 
Similarly, object nodes are added to the graph when previously undetected objects are detected.
}
\label{fig:episodicgraph}
\end{figure*}


==> fig/eval_example1.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=0.8\textwidth]{fig/eval_example1_.pdf}}\centering
\caption{
\textbf{Qualitative examples of navigation using SEA.}
% 
When given the goal object as a bed, the agent formulates a plan to navigate to the bedroom ($P_{12}$). To reach the bedroom ($P_{12}$), the agent predicts the subgoal place cluster using the categories of the initially visible objects.
% 
% \textbf{Row 1:} Initially, the agent estimates that the bedroom ($P_{12}$) is to the left, with the kitchen positioned directly ahead and to the right. It selects the left subgoal, anticipating that the target place is in that direction.
% % 
% \textbf{Row 2:} Upon reaching the subgoal, the agent commences a search for a bed, but fails to locate one. The agent then exits the area to identify a new subgoal. Given the visible door on the left, it deduces that the target place likely exists in that direction.
% % 
% \textbf{Row 3:} As the agent progresses towards the new subgoal, it detects the target object (a bed). The agent then devises a local plan to approach the target object. Finally, when the agent recognizes the matching place cluster as the searched-for bedroom ($P_{12}$), it activates the stop command.
% 
% We visualized more examples in the supplemental video.
} %\squeezeup
\label{fig:eval_example1}
\end{figure*}

==> fig/goal_ablation.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig/goal_ablation_.pdf}}\centering
\caption{
\textbf{Learning semantic relationships.}
% The figure provides an example demonstrating how SEA can identify efficient paths by leveraging semantic relationships. 
% % It depicts trajectories for six object goals: fireplace, cabinet, chair, chest of drawers, bathtub, and bed. 
% The trajectories of these six target object categories illustrate various pathways that are adapted according to the specific target object. 
% The starting point is symbolized by a yellow star, while a red region represents the goal boundary, which denotes that the goal is within a 1m radius.
The figure illustrates how SEA can identify efficient paths by leveraging semantic relationships. It shows the trajectories for six target objects: a fireplace, a cabinet, a chair, a chest of drawers, a bathtub, and a bed. These trajectories demonstrate various pathways that are adapted to each specific target object. The starting point is marked by a yellow star, while the goal boundary is represented by a red region, indicating that the goal is within a 1-meter radius.
% The starting point is marked with a yellow star, while the goal boundary, indicating that the goal is within a 1m range, is represented by a red region.
}
\label{fig:goal_ablation}
\end{figure*}

==> fig/image_encoder.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=\linewidth]{fig/image_encoder_.pdf}}\centering
\caption{
\textbf{Image encoder.} Figure showing the architecture of the image encoder.
}%\squeezeup\squeezelittle
\label{fig:image_encoder}
\end{figure*}%\squeezelittle


==> fig/intro.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=0.9\linewidth]{fig/intro_row.pdf}}\centering
\caption{
\textbf{Sub-problems in object goal navigation.}
% 
Given a task to find a microwave, 
% 
(a) infer the target location from the target object and determine the current  location using the current observation. 
% 
(b) Choose the most efficient semantic path from the current location to the target location. 
% 
(c) Discover the object by traveling to the desired location along the semantic path.
}%\squeezeup
\label{fig:intro}
\end{figure*}

==> fig/noise.tex <==
\begin{figure}[t!] %{0.5\textwidth}
\centering
\begin{minipage}{.4\textwidth}
\centering
\includegraphics[width=\textwidth]{fig/noise_.pdf}
\centering
\caption{\textbf{Ablation study on pose sensor noises.} SEA is robust on pose sensor noises.}%\squeezeup\squeezelittle
\label{fig:noise}
\end{minipage}
\end{figure}

==> fig/object_distribution.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig/object_distribution_1.pdf}}\centering
\caption{{Object distribution given a place cluster ($p(\mathbb{O}|\mathbb{P})$).}}
\label{fig:object_distribution_1}
\end{figure*}
\begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig/object_distribution_2.pdf}}\centering
\caption{{Object distribution given a place cluster ($p(\mathbb{O}|\mathbb{P})$).}}
\label{fig:object_distribution_2}
\end{figure*}
\begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig/object_distribution_3.pdf}}\centering
\caption{{Object distribution given a place cluster ($p(\mathbb{O}|\mathbb{P})$).}}
\label{fig:object_distribution_3}
\end{figure*}
\begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig/object_distribution_4.pdf}}\centering
\caption{{Object distribution given a place cluster ($p(\mathbb{O}|\mathbb{P})$).}}
\label{fig:object_distribution_4}
\end{figure*}

==> fig/object_encoder.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=\linewidth]{fig/object_encoder_.pdf}}\centering
\caption{
\textbf{Object encoder.} Figure showing the architecture of the object encoder.
}%\squeezeup\squeezelittle
\label{fig:object_encoder}
\end{figure*}%\squeezelittle


==> fig/object_importance.tex <==
\begin{figure*}[ht]{\centering\includegraphics[width=\textwidth]{fig/object_importance_.pdf}}\centering
\caption{Illustrating the significance of objects in distinguishing and identifying individual place clusters.}
\label{fig:object_importance}
\end{figure*}

==> fig/overview.tex <==
\usepackage{graphicx}
\begin{figure*}[t!]{\includegraphics[width=\textwidth]{fig/overview_.pdf}}
\caption{
\textbf{Overview of semantic environmental atlas (SEA).} 
% 
The semantic graph map (SGM) is updated using visual observations. %: an episodic graph, semantic prior graph, global policy, and local policy.
% 
% An episodic graph encodes semantic relationship using the sequence of observations.
% 
Then, the place relationship and place-object connections across environments are updated using multiple semantic graph maps collected from different environments.
% 
A global policy samples a subgoal $g_t$, which is reachable and most likely to be near to the target place.
% 
A local policy generates navigational actions to reach the subgoal. 
% 
}
% See text for more details.
\label{fig:overview}
\end{figure*}

==> fig/place_connection.tex <==
\begin{figure*}[h!]{\centering\includegraphics[width=\textwidth]{fig/place_connection_.png}}\centering
\caption{
\textbf{Formation of Semantic Graph Map from Training Environments.} The figure illustrates the process of forming a semantic graph map from multiple training environments.
In each training environment, it checks to see whether there is a pair of place clusters.
% 
If there a connection between the pair of places, the reachability is set to one; otherwise, zero.
}
\label{fig:place_connection}
\end{figure*}

==> fig/place_distribution.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig/place_distribution_1.pdf}}\centering
\caption{{Place distribution given an object category ($p(\mathbb{P}|\mathbb{O})$).}}
\label{fig:place_distribution_1}
\end{figure*}
\begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig/place_distribution_2.pdf}}\centering
\caption{{Place distribution given an object category ($p(\mathbb{P}|\mathbb{O})$).}}
% \caption{{Object distribution given place clusters ($p(\mathbb{O}|\mathbb{P})$).}}
\label{fig:place_distribution_2}
\end{figure*}
\begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig/place_distribution_3.pdf}}\centering
\caption{{Place distribution given an object category ($p(\mathbb{P}|\mathbb{O})$).}}
% \caption{{Object distribution given place clusters ($p(\mathbb{O}|\mathbb{P})$).}}
\label{fig:place_distribution_3}
\end{figure*}

==> fig/place_encoder.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=\linewidth]{fig/place_encoder_.pdf}}\centering
\caption{
\textbf{Place encoder.} Figure showing the architecture of the place encoder.
}%\squeezeup\squeezelittle
\label{fig:place_encoder}
\end{figure*}%\squeezelittle


==> fig/place_reachability.tex <==
\begin{figure}[t!]{\centering\includegraphics[width=0.9\linewidth]{fig/place_reachability_.pdf}}\centering
\caption{
\textbf{Construction of place-to-place prior graph.}
% 
In each training environment, it checks to see whether there is a pair of place clusters.
% 
If there a connection between the pair of places, the reachability is set to one; otherwise, zero.
% 
If there are three environments where two places are found, and they are connected twice, the reachability between two places are $r_{ij}$ = 2/3, where a bedroom is $i$th place and a bathroom is $j$th place.
}
\label{fig:place_rechability}
\end{figure}

==> fig/place_reachability_matrix.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig/place_reachability_matrix_.pdf}}\centering
\caption{ \textbf{Reachability of places.} The place clusters designated for the hallway, indicated by the {\color{darkred}\textbf{red}} box, have links to numerous other places, suggesting that the hallway serves as a bridge between different places.
% 
The clusters associated with the kitchen are strongly connected to other kitchen types (denoted by the {\color{darkgreen}\textbf{green}} box) or dining rooms (highlighted in the {\color{darkorange}\textbf{orange}} box).
% 
This illustrates that reachability is at one when place clusters are adjacent, whereas the connectivity between distant place clusters yields a reachability of zero.}
\label{fig:place_reachability_matrix}
\end{figure*}

% The place clusters for the hallway (see {\color{darkred}\textbf{red}} box) are linked to many other places, which means that the hallway is a bridge between places.
% % 
% The kitchen clusters are highly associated to other types of kitchens ({\color{darkgreen}\textbf{green}} box) or dining rooms ({\color{darkorange}\textbf{orange}} box).
% % 
% It demonstrates that reachability is one when place clusters are adjacent and the connectivity between distant place clusters has zero reachability.
% visualization을 위해 x축을 절반으로 잘라서 아래에 붙였다.
% hallway ($P_{26}, P_{44}$) 는 대부분의 다른 place들과 연결된 것을 볼 수 있고, 
% kitchen ($P_{24}$)은 다른 종류의 kitchen ($P_{13}$, 0.43, $P_{22}, 0.48$) 또는 dining table ($P_{23}$, 0.44)과 연결성이 높은 것을 확인 할 수 있다.
% 
% }
% \label{fig:place_reachability_matrix}
% \end{figure}
% \begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig/place_reachability_part2.pdf}}\centering
% \caption{place reachability visualize}
% \label{fig:place_reachability_part2}
% \end{figure*}

==> fig/semantic_planning.tex <==
\begin{figure*}[t!]{\centering\includegraphics[width=\textwidth]{fig_supp/semantic_planning_.pdf}}\centering
\caption{
\textbf{Analysis on the semantic path planning.}
Assume the current place cluster $P_t$ is a dining room and the goal object to be a toilet.
% 
% The target place cluster $P_{k^*_t}$ can be estimated using the target object.
% 
A shortest semantic path, $\Tau^* = \{P_{\tau_1}, P_{\tau_2}, P_{\tau_3}, P_{\tau_4}\}$ is generated, where $P_{\tau_1}$ is the current place cluster (dining room) and $P_{\tau_4} = P_{k^*_t}$ is the estimated target place (bathroom).
% 
The place names indicate the ground truth place obtained from the training scenes. 
% 
% The map's hue represents the likelihood of the place cluster would be exist in the place.
The colored maps are red when the similarity to the place cluster is high and gets blue when there is a low similarity.
% 
% The color is red when the likelihood is high and gets blue when there's a low chance the place cluster exists.
% 
The red box denotes the area where the corresponding place cluster is most likely to exist in the environment, and the arrow denotes the path that could be moved using semantic path planning.
% 
The results are extracted from the prior distributions, without updating.
% 
The colors and the cut-out maps are used for visualization purposes only. 
Full visualization is in Section 3 of the supplementary material.
}%\squeezeup
\label{fig:semantic_planning}
\end{figure*}


==> fig/subgoal_selection_example.tex <==
\begin{figure}[h!]{\centering\includegraphics[width=0.5\linewidth]{fig_supp/subgoal_selection_example_.pdf}}\centering\squeezelittle\squeezelittle
\caption{\scriptsize\squeezelittle
{Example of selecting a subgoal location.}
}\squeezeup
\label{fig:subgoal_selection_example}
\end{figure}

==> fig/training_cost.tex <==
\begin{figure}[t!]
\begin{minipage}{.45\textwidth}{
\centering
\includegraphics[width=\textwidth]{fig/training_cost_.pdf}
}
\centering
\caption{{Training cost on MP3D.}}
\label{fig:training_cost}
\end{minipage}
\end{figure}
\squeezeup
% [width=\linewidth]
